ECMO: Peripheral Transplantation to Rehost Embedded Linux Kernels

Dynamic analysis based on the full-system emulator QEMU is widely used for various purposes. However, it is challenging to run firmware images of embedded devices in QEMU, especially the process to boot the Linux kernel (we call this process rehosting the Linux kernel.) That's because embedded devices usually use different system-on-chips (SoCs) from multiple vendors and only a limited number of SoCs are currently supported in QEMU. In this work, we propose a technique called peripheral transplantation. The main idea is to transplant the device drivers of designated peripherals into the Linux kernel. By doing so, it can replace the peripherals in the kernel that are currently unsupported in QEMU with supported ones, thus making the Linux kernel rehostable. After that, various applications can be built upon. We implemented this technique inside a prototype system called ECMO and applied it to 815 firmware images, which consist of 20 kernel versions, 37 device models, and 24 vendors. The result shows that ECMO can successfully transplant peripherals for all the 815 Linux kernels. Among them,710 kernels can be successfully rehosted, i.e., launching a user-space shell (87.1% success rate). The failed cases are mainly because the root file system format (ramfs) is not supported by the kernel. We further build three applications, i.e., kernel crash analysis, rootkit forensic analysis, and kernel fuzzing, based on the rehosted kernels to demonstrate the usage scenarios of ECMO

==> evaluation.tex <==
\section{Evaluation}

In this section, we present the evaluation result of \sysname. We first introduce our dataset. Then we evaluate \sysname by answering the following three questions.

\begin{itemize}
    %\item Is \sysname available to rehost the Linux Kernel without the source code? 
    \item \textbf{RQ1:} Is \sysname able to identify the \code{\sysname Pointers} ?
    \item \textbf{RQ2:} Is \sysname able to re-host the Linux kernel of embedded devices in different Linux kernel versions, different vendors, and different device models?
    \item \textbf{RQ3:} What is the functionality of Linux kernel rehosted by \sysname?  Is the provided functionality able to conduct security analysis (e.g., crash analysis, rootkit forensic analysis, and fuzzing)?
\end{itemize}


\subsection{Dataset}
As we target on re-hosting the Linux kernel of embedded devices, we collect the firmware images from both the third party projects (i.e., OpenWRT~\cite{openwrt}) and the official vendors (i.e., Netgear~\cite{Netgear} ).
Due to the popularity of ARM architecture in embedded devices~\cite{arm_roadshow}, our evaluation targets on Linux kernel in ARM devices. However, the overall mechanism can also be applied to other architectures (e.g., MIPS).
%Meanwhile, we ignore the firmware images whose CPU types are not supported by \code{QEMU}. 
%Supporting more CPU series is a valuable question but out of our scope.

We transplant three key peripherals (i.e., IC, timer, and UART). 
For IC, we use PrimeCell Vectored Interrupt Controller (PL190)~\cite{pl190}.  For timer, we use ARM Dual-Timer Module (SP804)~\cite{sp804}. The other IC and Timer can also be transplanted. For UART, we noticed that 77\% of firmware images in OpenWRT support the UART ns16550. We reuse the driver of ns16550 and only transplant the peripheral model.
%To If we want to finally have the shell, an appropriate UART is required. We ignore the firmware whose UART are not supported by QEMU.
In total, we collect 1006 firmware images. We use \code{Preprocessor} to unpack the downloaded firmware. Among them, 824 firmware images (720 in OpenWRT and 104 in Netgear) contain Linux kernels while the left 182 ones only contain file systems, which are excluded from our evaluation.
%We further explore the 720 firmware images and find that they cover 32 different SoCs and can be applied to devices from 24 different vendors.  We will detail the evaluation results in the following sections.

\subsection{Identify ECMO Pointers (RQ1)}
\input{table/pointer2}
%As we mentioned before, to transplant peripherals, we have to identify the right \sysname pointers. Otherwise, the transplanted peripheral cannot communicate with the original Linux kernel successfully. 
\code{\sysname Pointers} are important to \textit{peripheral transplantation}.
In this section, we evaluate the success rate on identifying \code{\sysname Pointers}. 
%Note that different Linux kernel versions provide different APIs for the transplanted peripheral to use.
Among all the 824 Linux kernels, there are 17 different kernel versions.
Table~\ref{tab:pointer} lists the required \code{\sysname Pointers}, the strategies we use, and the description of these \code{\sysname Pointers}. In total, we need to identify 24 different \code{\sysname Pointers} for all the 17 Linux kernel versions. Among all the 24 \code{\sysname Pointers}, two of them (i.e., \textit{mach\_desc-\textgreater{}init\_time}, and \textit{mach\_desc-\textgreater{}init\_irq} ) are data pointers. Identifying the data pointers is rather more difficult than identifying the function pointers as we need to identify symbols in each function and infer the right ones. However, the data pointer \textit{mach\_desc-\textgreater{}init\_time}, and \textit{mach\_desc-\textgreater{}init\_irq} can be calculated directly from the return value of \textit{setup\_machine\_fdt} or \textit{lookup\_machine\_type}.
 
%For the left data pointer (i.e.,\textit{cpu\_possible\_mask}),
%we manually study the usage of this data pointer and find that this pointer will be used to check the CPU status while registering timer. Thus, we set the value of this pointer as the address that we can control and feed the expected value (i.e., 1, which means CPU 1) to the address that the data pointer points to. 
In this case, we only need to identify 22 \code{\sysname Pointers} and all of them are function pointers. Among all the 22 \code{\sysname Pointers}, 7 are identified with strategy three, which demonstrates the necessity of our three policies.

\input{table/disa}
Identify \code{\sysname Pointers} requires us to disassemble the decompressed Linux kernel.
Table~\ref{tab:disa} lists the statistics of disassembly. 
%The firmware image is about 460k bytes in average while the unpacked uImage is about 177k bytes in average. 
The decompressed Linux kernel is about 868k bytes on average. With \code{Pointer Analyzer}, the Linux kernel can be disassembled and more than 20 thousand functions are generated. Though there might be many false positives in the located functions, it contains all our required  \code{\sysname Pointers}. Among the more than 20 thousand functions, we can 100\% identify all our required \code{\sysname Pointers} for all the Linux kernels.



\input{table/overall}

\subsection{Rehost Linux Kernels (RQ2)}
In this section, we evaluate the capabilities of \sysname on re-hosting the Linux kernel. 

\subsubsection{Firmware Images from Third Party Projects}

Table~\ref{tab:overall} shows the overall result and the success rate of \textit{peripheral transplantation} and re-hosting for OpenWRT. We define the success \textit{peripheral transplantation} as that the timer can trigger interrupts periodically, the IC can handle the interrupts by switching between \code{irq} mode and \code{svc} mode, and the UART can print the boot message in the console.
If the Linux kernel enters into the user-space and spawns a shell, then we treat it as a successful re-hosting.
%
%We define the success re-hosting as that the Linux kernel can enter into \code{user} mode and we can obtain the shell.

\smallskip
\noindent \textbf{Linux Kernel Version} 
%In overall, we have 902 firmware images and we can unpack all of them with our patched \code{binwalk}. 720 of 902 contain the Linux kernels. 
The kernels in the 720 firmware consist of  16 different kernel versions. As we mentioned before, we can successfully identify all the required \code{\sysname Pointers}. With  \code{\sysname Pointers}, our evaluation shows that we can transplant the IC, timer, and UART for all the 720 Linux kernels successfully. We noticed that some of the Linux kernels cannot be rehosted. This is because these Linux kernels cannot recognize our pre-built root file system. Without the root file system, we cannot get the shell. Linux kernels in 4.14.x version do not have such problems. To conclude, we can transplant peripherals for all the 720 firmware images and rehost 86.7\% of them. 

\smallskip
\noindent \textbf{Vendor} \sysname can rehost the Linux kernels of embedded devices for 24 different vendors. Figure~\ref{fig:vendor} shows the result. We list the top five vendors that produce most Linux kernels. We notice that \code{Netgear}, \code{Asus}, \code{Pogoplug}, \code{Buffalo}, and \code{Linksys} are among the top five vendors in the OpenWRT dataset. Among them, \code{Pogoplug} has a relatively low success rate of re-hosting. Most of the Linux kernel from the vendor in \code{Pogoplug} cannot recognize our pre-built root file system.

\begin{figure}[t]
\centering
\includegraphics[scale=0.45]{figures/vendor.pdf}
\caption{Vendor Distribution of Linux Kernels.}
\label{fig:vendor}
\end{figure}


\smallskip
\noindent \textbf{Device Model} We extract the Device model information from the unpacked \code{DTB} file. We decompile the \code{DTB} file to \code{DTS} file and collect the \code{compatible} value in the root node. One \code{compatible} value is seen as one device model. Overall,
\sysname can rehost the Linux kernels of embedded devices from 32 different device models. We notice that all the Linux kernels that cannot be rehosted by \sysname are from the device model \code{"plxtech,nas7820/nas782x"}. This type of device model includes 144 Linux kernels. We can transplant peripherals to all of these Linux kernels. However, only 48 of them can recognize our pre-built root file systems. The left 96 cannot be rehosted as they cannot recognize our pre-built root file system.

\input{table/netgear}
\subsubsection{Firmware Images from Official Vendors}
We also apply \sysname on the firmware images released by vendors (i.e., Netgear). We collect all the firmware images for five popular devices (i.e., R6250, R6300v2, R6400, R6700, R6900). Table~\ref{tab:netgear} shows the result. We noticed that all the Linux kernels of Netgear are in version 2.6.36. Since Linux kernel in version 2.6.36 does not support DTB, we think the five different popular devices can be seen as five device models. We can successfully transplant the peripherals to all the 104 different firmware images. Among the 104 firmware images, we can launch the shell for 95 ones while the left 9 cannot be rehosted due the the file system problems.



\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/root_cause.pdf}
	\caption{CVE-2016-9793: The root cause is Type Confusion Error. Type \code{u32} results in a negative return value and it should be changed into type \code{int}.}
	\label{fig:root_cause}
\end{figure}




\subsection{Conduct Security Analyses (RQ3)}
\smallskip
\noindent \textbf{Functionality} In this section, we evaluate the  functionality and usage of Linux kernel rehosted by \sysname. We first evaluate the basic functionality of the rehosted Linux kernel with a syscall testing tool in LTP (Linux Test Project~\cite{ltp}). After that, we demonstrate the usage and functionality of the rehosted Linux kernel with three different kinds of security applications (i.e., crash analysis, rootkit forensic analysis, and fuzzing).

In total, we run 1270 syscall test cases on the rehosted Linux kernel. 148 of them are skipped as the testing environment (e.g., architecture, build configuration) does not meet the requirement. In the left 1122 test cases, 944 test cases passed while the left 178 ones are failed. We further analyze the test cases and find that the passed test cases cover the fundamental functionalities (e.g., task management, memory management, and virtual file systems) of the Linux kernel. For the failed ones, most of them aim to test the robustness and security of the Linux kernel. For example, LTP tests whether the kernel fix the specific vulnerabilities (i.e., CVE-2017-18344~\cite{CVE-2017-18344}). If the tested Linux kernel does not fix the 

\subsubsection{Crash Analysis}
Crash analysis is very important as it can save a lot of time for developers to patch the bugs and protect the software (e.g., Linux kernel). However, it is rather hard to understand the root cause without dynamic analysis.
First, they cannot do debugging if they do not have real devices. Second, even they can run the Linux kernel on real devices, they cannot obtain the run time trace, which can increase the difficulty of debugging. 
We utilize \sysname to conduct crash analysis (i.e., understand the root cause of the crash) on the rehosted Linux kernels. 
Table~\ref{tab:cve} lists 6 different kinds of 1-day CVEs and \sysname can successfully trigger all of them and understand their root cause. These CVEs cover five different CVE types and some of them have relatively high scores (e.g., 7.8), which are defined in the National Vulnerability Database~\cite{nvd}.
\input{table/cve}
We detail the procedures on how to conduct crash analysis with one CVE (CVE-2016-9793~\cite{cve_2016-9793}), which has a very high CVE score (7.8), triggered by \sysname. After re-hosting the Linux kernel successfully, we can launch the shell and trigger the vulnerability. We then dump all the run time trace collected by \code{QEMU}.



Figure~\ref{fig:root_cause} shows how \sysname can help us understand the root cause of CVE-2016-9793. When the rehosted Linux kernel crashes, the detailed call stack will be printed out. The call stack includes the function name and the addresses of these functions. 
Since we can collect the trace during the re-hosting process, we can map the trace to the call stack. With the trace, we can get the run time information including the register value and execution path.
By analyzing the trace, we are able to locate the parameters for each function. We noticed that a negative value (i.e., \code{0xffffff40}) is the first parameter of function \textit{\_\_alloc\_skb}. This negative value results in crash. We analyze the propagation of this negative value with the trace. We noticed that this value is propagated by the first parameter of function \textit{sock\_alloc\_send\_pskb}. Finally, we noticed that the negative value \code{0xffffff40} is calculated from \code{0xffffff00}, which is loaded in function \textit{unix\_stream\_sendmsg} from address \code{0xc7929110}. We use \code{GDB} to set a watchpoint at this address. It is easy to find that instruction \code{0xc0229f68} is writing the negative value (i.e., \code{0xffffff00} ) into address \code{0xc7929110}. \code{Pointer Analyzer} can help us to identify the function that contains the instruction \code{0xc0229f68}.
By analyzing the function, we find that the root cause of the crash is because of type confusion error. In function \textit{sock\_setsockopt}, the variable \textit{sk	$\rightarrow$sk\_sndbuf} will be set by the return value of \textit{max\_t}. However, due to the wrong type \code{u32}, the return value can be a negative value. Furthermore, this vulnerability can be exploited to compromise Linux kernel. Attackers can control this device via this vulnerability and launch severe attacks. 
Thus, we patch the vulnerability by changing the type \code{u32} to \code{int}. If we do not have \sysname, we cannot rehost the corresponding Linux kernel. When there is a vulnerable input that can crash the target kernel, it is rather difficult for developers to locate the root cause. This demonstration shows the usage of \sysname.

\subsubsection{Rootkit Forensic Analysis}
Rootkit forensic analysis requires the ability to monitor the run time state of the kernels (i.e., Virtual Machine Introspection(VMI)~\cite{garfinkel2003virtual}). We demonstrate this ability of \sysname by conducting rootkit forensic analysis with one (i.e., \textit{Suterusu}~\cite{suterusu})  of the very popular rootkits in the wild. 

\textit{Suterusu}  is able to hide the specific process ID by hijacking the kernel function \textit{proc\_readdir}, which is used to get the process information. Figure~\ref{fig:rootkit_flow} shows how \textit{Suterusu} works. 
It will hijack the function \textit{proc\_readdir} by rewriting. \textit{Suterusu} will rewrite the function \textit{proc\_readdir}'s first instruction by instruction \code{LDR PC,[PC,\#0]} to redirect \textit{proc\_readdir} to the self-defined function \textit{new\_proc\_readdir}. Thus, \textit{Suterusu} can successfully hide the specific process. With \sysname, we can monitor the code section after the Linux kernel is rehosted by setting watchpoints, which is shown in Figure~\ref{fig:rootkit_gdb}. Once we noticed that the code section is rewritten, the kernel may be attacked by the rootkit.


\begin{figure}[t]
  \centering

  \subfigure[Workflow of rootkit \textit{Suterusu}]{\includegraphics[width=0.22\textwidth]{figures/rootkit.pdf}\label{fig:rootkit_flow}}
  \subfigure[\sysname observes how the rootkit \textit{Suterusu}  works. ]{\includegraphics[width=0.22\textwidth]{figures/rootkit_gdb.pdf}\label{fig:rootkit_gdb}}

  \caption{The workflow of rootkit  \textit{Suterusu} and how \sysname can analyze the behavior}
  \label{fig:rootkit}

\end{figure}


\subsubsection{Fuzzing}
Fuzzing technique is a widely used and effective technique to detect the software vulnerabilities. Given one problem, we have to provide the run time environment and the capability of monitoring the coverage information. \sysname can provide both of these two pre-requirements by emulating. We demonstrate the capability of \sysname by integrating one of the most popular kernel fuzzers (i.e.,\code{UnicornFuzz}~\cite{maier2019unicorefuzz}). Note that the fuzzing technique and whether it can find new vulnerabilities are out of this paper's scope. We integrate the \code{UnicornFuzz} into \sysname and continuously fuzz the example kernel modules provided by \code{UnicornFuzz} for one hour. We observed that the \code{UnicornFuzz} can work normally  and the execution speed can reach to 390 per second, which demonstrate the usage and functionalities of \sysname.

==> implementation.tex <==
\section{Implementation}

We implement \sysname based on \code{QEMU}.
We first port \code{LuaQEMU}~\cite{luaqemu} to support the newer version of \code{QEMU}.
\code{LuaQEMU} is a framework based on \code{QEMU} and it can exploit several \code{QEMU} internal APIs to LuaJIT~\cite{LuaJIT}. With \code{LuaQEMU}, we are able to set breakpoints during the re-hosting process of Linux kernel and dynamically read/write registers/memory at the breakpoints. We further exploit more internal APIs to initialize the model of peripherals (hardware). 
%As LuaQEMU provides interface to read/write the value in memory/registers. We write Python script to automatically generate the Lua script for the different purpose.

As for the \sysname modules,
\code{Preprocessor} is implemented based on \code{binwalk}~\cite{binwalk}. We patch \code{binwalk} to support more formats. With \code{binwalk}, we can dump the required \code{zImage} of Linux kernel. We use \code{mkimage}~\cite{mkimage} to add the required u-boot information on \code{zImage} to generate \code{uImage}. 
%As for \code{DTB}, we utilize the Python \code{fdt} module~\cite{fdt} to inject the description of peripherals into \code{DTB}.

\code{ Decompressor} is implemented based on \code{LuaQEMU} with some glue scripts in Python. 
We set up a breakpoint after the function \textit{setup\_machine\_fdt} returns and dump the decompressed kernel by reading the specific memory space via \code{Lua} script. 
\code{Driver Generator} and \code{Pointer Analyzer} are both implemented by Python scripts. 
As the \code{Driver Generator} is responsible for generating and selecting  \code{\sysname Driver}, we write \code{\sysname Driver} in c code manually and cross-compile it with GCC. Note that this is one-time effort. One \code{\sysname Driver} is able to be used by Linux kernels in several different kinds of versions if they all have the required \code{\sysname Backward Pointers}. 
For \code{Pointer Analyzer}, we utilize \code{Capstone}~\cite{capstone} to disassemble the decompressed Linux kernel..
As for the partial emulation, we utilize \code{Unicorn}~\cite{unicorn}. In total, we have around 2,880 lines of Python code.

%For the interrupt controller, we use PrimeCell Vectored Interrupt Controller (PL190)~\cite{pl190}. The other interrupt controller can also be transplanted. For the timer, we use PrimeCell Vectored Interrupt Controller (SP804)~\cite{sp804}.





==> introduction.tex <==
\section{Introduction}
Embedded devices are becoming popular. 
%The market of IoT devices is projected to reach more than 150 billion in 2024~\cite{iot_market}.
Many of them run Linux-based operating systems.
According to the vulnerability statistics of Linux kernels~\cite{cve_kernel}, hundreds of vulnerabilities are explored every year. 
%Nearly half of the vulnerabilities can be abused to conduct DDoS (Distributed Denial of Service) attacks.
Once the operating system (i.e., Linux kernel) of the embedded devices is compromised, attackers can control billions of compromised devices. 
%For example, Mirai botnets compromised millions of embedded devices to conduct the DDoS attack,
%disrupting the Internet service and resulting in a huge loss~\cite{mirai_news3, mirai_news2, mirai_news1}.
Thus, the security of embedded devices, especially the Linux kernel, deserves a thorough security analysis. 
% attention. 

Dynamic analysis are widely used to conduct security analysis~\cite{rept2020atc,cui2018rept}. This is because dynamic analysis is precise and can monitor the run time behavior while static analysis~\cite{redini2020karonte,shoshitaishvili2015firmalice,UsenixSec14_Costin, hernandez2017firmusb} cannot. To support dynamic analysis, we have to provide the capability to \textit{introspect the run time states of the target programs}. Re-hosting, also known as emulating, is proposed to provide this capability.
 %In other words, the capability of emulation. 
 Based on this capability, we can build different kinds of security applications (e.g., crash analysis, rootkit forensic analysis, and fuzzing) to conduct different security analysis.

Previous work (i.e., \code{FIRMADYNE}~\cite{chen2016firmadyne}) provides the capability of re-hosting for user-space programs with the help of a customized kernel. However, different from user-space programs, Linux kernel of embedded device is not easy to be emulated due to the various peripherals. Researchers utilize real devices~\cite{zaddach2014avatar,avatar2,eric2019pretender,talebi2018charm} to solve the peripheral dependency problems, but these mechanisms are not scalable as there exist thousands of different devices. Other solutions target bare-metal systems~\cite{feng2019p2im,dice,clements2019hal} and the mechanisms can not be applied to emulate the Linux kernel of embedded devices. Thus, re-hosting Linux kernel of embedded devices at scale is still an unsolved problem.


%Previous studies applied the static analysis~\cite{redini2020karonte,shoshitaishvili2015firmalice,UsenixSec14_Costin, hernandez2017firmusb} on the security issues of embedded devices. However, static analysis has limitations. Security analysis such as locating the root cause of vulnerabilities and virtual machine introspection~\cite{garfinkel2003virtual} cannot be conducted via static analysis.
%To complement it, the re-hosting technique that performs the dynamic analysis with the help of an emulator is proposed.
%Due to the diverse peripherals in embedded devices,
%state-of-the-art full system emulators (e.g., \code{QEMU}~\cite{bellard2005qemu}) only support limited devices.
%Some studies utilize real devices~\cite{zaddach2014avatar,avatar2,eric2019pretender,talebi2018charm}.
%However, they are not scalable as there exist thousands of different devices.
%Besides, it's challenging to collect the run-time information on real devices.
%Other works~\cite{feng2019p2im,dice,clements2019hal,harrison2020partemu} are proposed to support
%scalable emulation of embedded devices. They either target bare-metal systems or
%user-level programs. Re-hosting Linux kernels of embedded devices is still an open research problem.



%\smallskip
%\noindent \textbf{Challenges:}
%There are three main challenges on re-hosting the Linux kernel of embedded devices.First, without the right peripheral model, the Linux kernel may crash, get stuck in an infinite loop,or exit during the re-hosting process. Second, peripherals vary a lot. It is rather hard to build a general model for all kinds of peripherals. Third, most of the Linux kernels of embedded devices are stripped. This brings obstacles as the peripheral model is hard to be inferred from stripped binaries.

%\smallskip
%\noindent \textbf{Observations}: To address the above mentioned three challenges, we carefully study the Linux kernel and have three important observations. For the first challenge, we observe that not all peripherals need to be emulated for the re-hosting task and we only need to guarantee the functionality of key peripherals. For the second challenge, Linux kernel provides interfaces to implement drivers of these peripherals, which brings the chance to replace these diverse peripherals with designated ones. For the third challenge, Linux kernels of different devices share most of the code, which is open-source.




\smallskip
\noindent \textbf{Our Approach}: To rehost the Linux kernel of embedded devices, we propose a novel technique called \textit{peripheral transplantation} that is \textit{device-independent} and has no assumption of available source code. \textit{Peripheral transplantation} aims to transplant designated peripherals into the target Linux kernel.
It replaces the peripherals that are currently not supported by the state-of-the-art full system emulator (i.e., \code{QEMU})
with support ones. With the transplanted peripherals, \code{QEMU} can successfully rehost the
Linux kernel. Analysts can build different security applications based on the re-hosted Linux kernel afterwards.




\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/ecmo_intro_new.pdf}
    \caption{The overview of our framework.}
    \label{fig:ecmo_intro}
  \end{figure}

%To transplant the customized peripheral and make it work, we have to transplant the driver of the peripheral (software) and the model of the peripheral (hardware). Transplanting the model of peripheral is intuitive as the host (i.e., \code{}) is controlled by ourselves. 



  
%The market of IoT devices is projected to reach more than 150 billion in 2024~\cite{iot_market}. 
%ARM is the dominant architecture for IoT controllers with more than $90\%$ of the market share~\cite{arm_roadshow}. As such, this paper focuses on the ARM architecture but its methodology can be applied to other architectures as well. 

% current works focus on linux-based. user-level 
% cannot solve linux-based.
%Previous works used to target on bare-mental systems~\cite{clements2019hal,feng2019p2im,dice} or  user-space programs~\cite{chen2016firmadyne,redini2020karonte}. However, few works target on the Linux based operating systems and focus on the kernel security. With the increasing size of the Linux kernel source code, the number of the vulnerabilities keep growing. The security issue of Linux kernel deserves our attention.


% static analysis has limitations. we need to do dynamic analysis. there are challenges in dynamic analysis. thus, we need to emulate. 
%challenges of emulation
%our approach.
%However, the software of these devices (i.e., firmware) used to be closed-source. Without source code, researchers have to conduct binary analysis on the proposed firmwares. Mechanisms of binary analysis can be divided into two different types. They are static analysis and dynamic analysis. 

% Dynamic/Static analysis can reduced.
%Dynamic analysis is accurate with high confidence. To conduct dynamic analysis, some studies utilize the real devices~\cite{zaddach2014avatar,avatar2}. However, it is not scalable as we can not collect all the real devices. Furthermore, we cannot obtain the run time information with real devices.
%Other works~\cite{feng2019p2im,dice,clements2019hal,harrison2020partemu} build models to support different peripherals to conduct dynamic analysis. However, neither of these work targets on emulating the Linux kernel of embedded devices. 
% explain why closed source is challenge
% Our Goal.
% We have some observations to overcome the above mentioned challenges 1.2.3 - observation 1.2.3 should be matched. connect with the pre-mentioned challenges.

% 注意时态，全部用现在式； 在正文最好都用现在式
% what does controlled by ourselves mean? Why it is intuitive? 尽量不要用intuitive/trivial 等词汇. 
\textit{Peripheral transplantation} needs to transplant two components, i.e., emulated model
of the peripheral (into \code{QEMU}) and the driver of the peripheral (into the Linux kernel).
Transplanting the peripheral model requires us to build the hardware emulation code for a
specified (or simplified) peripheral and integrate it into \code{QEMU}.
We utilize APIs provided by \code{QEMU} for transplanting emulated peripheral models.
Transplanting the driver into the Linux kernel is non-trivial since we have to achieve three
design goals: \emph{First}, the code of the transplanted driver should be position-independent.
Otherwise, the \textit{peripheral transplantation} technique is limited by the loading address of
the transplanted driver. 
\emph{Second}, the transplanted driver should not affect the memory view of the Linux kernel.
Otherwise, the memory space storing the transplanted driver can be overwritten by the Linux kernel (since
the kernel is not aware the existence of the driver), resulting in crashes.
\emph{Third}, the transplanted driver needs to communicate with the original Linux kernel.
Otherwise, the transplanted driver cannot be initialized and its functionality cannot be guaranteed. 

%by the Linux kernel and the driver cannot configure the peripheral models. % Add reasons for each challenge.



To solve these challenges, 
we implement and integrate the \textit{peripheral transplantation} technique into
\code{QEMU} to create a firmware dynamic analysis platform called \sysname. We detail our design in Section~\ref{sec:solution}. 
Figure~\ref{fig:ecmo_intro} shows the basic workflow of \sysname. \sysname receives the firmware image and the peripherals to be transplanted. \sysname will transplant the peripherals to the Linux kernel in the firmware image. 
%The transplantation process helps to break the limitation of peripheral fragmentation. % fragmentation -> diversity ? break ? a unified approach to solve the problem due to the diversity of peripherals.
After transplanting the peripherals, the Linux kernel will be re-hosted successfully to launch a shell.
Then we can conduct security analysis based on the re-hosted Linux kernel of embedded devices.
%We observed that the key challenge of rehosting the linux kernel are the variaty of interrupt controller and timer. We design and build a general pair of interrupt controller and timer. With the abstraction of linux kernel, we then inject our self-compiled interrupt controller and timer into the original linux kernel with dynamic binary rewriting techniques. As the interrupt controller and timer are built by ourselves, we prepare a matched hardware emulator of these two components and integrated them into \code{QEMU}. 


%Since ARM is the dominant architecture for IoT controllers with more than $90\%$ of the market share~\cite{arm_roadshow}, this paper focuses on the ARM architecture. 
%However, its methodology can be applied to other architectures (e.g., MIPS) as well. 
We apply \sysname on 815 Linux kernels that are extracted from different kinds of firmware images including 20 different kernel versions, 37 device models, and 24 vendors. Our experiments show that \sysname can successfully transplant peripherals on all the 815 Linux kernels. Among them, 710 can be re-hosted to launch a shell.
To demonstrate the functionality and usage of \sysname, we build three different kinds security applications (i.e., crash analysis, rootkit forensic analysis, and fuzzing) based on the rehosted Linux kernel.
%successfully trigger six 1-day CVEs on the Linux kernel re-hosted by \sysname. % one of the motivation. We detail the analyzing process on one severe vulnerability and find that \sysname can help us locate the root cause of the vulnerability. Furthermore, we apply \sysname to conduct virtual machine introspection. Our experiments shows that \sysname can realize the existence of rootkits and understand how they work.

Overall, this work makes the following main contributions.
\begin{itemize}
    \item \textbf{Novel Technique}\tab We propose a \textit{device-independent}  technique (i.e., \textit{peripheral transplantation}) that can re-host the Linux kernels of embedded devices without the availability of its source code.
    \item \textbf{New Tool}\tab We implement and integrate the \textit{peripheral transplantation} technique into \code{QEMU}, to create a new firmware dynamic analysis platform called \sysname.
    \item \textbf{Comprehensive Evaluation}\tab We apply \sysname to Linux kernels from 824 different images.
    \sysname can transplant peripherals for all the Linux kernels and successfully launch the shell for 719 ones.
    Furthermore, we build three different kinds security applications (i.e., crash analysis, rootkit forensic analysis, and fuzzing) based on the rehosted Linux kernel, which demonstrate the usage and functionality of \sysname.
    
  \end{itemize}

To engage the community, we will release all the source code of our system.

==> mechanism.tex <==
\section{Overall System Design}

\subsection{Challenges}
Re-hosting the Linux kernel of embedded devices is not easy. To conclude, 
there are three main challenges in re-hosting the Linux kernel of embedded devices. 

\smallskip
\noindent \textbf{Peripheral Dependence}: Re-hosting the Linux kernel of embedded devices requires solving peripheral dependence.  Different embedded devices have different peripherals.
Linux kernels access these peripherals  via the MMIO (Memory-Mapped I/O) mechanism.
Specifically, the hardware registers of peripherals are mapped into the normal address space and accessed via memory load and store instructions.
Without the right peripheral model,
the Linux kernel may crash, stuck in an infinite loop, or exit during the boot process.
Thus, we have to provide the right peripheral models in \code{QEMU}.
The right model not only needs to guarantee that the Linux kernel can be re-hosted,
but also needs to support the functionality of these peripherals. 
%However, without the source code or specification of these peripheral, it is hard to infer the memory addresses of these peripherals and their semantics.

\smallskip
\noindent \textbf{Peripheral Diversity}: Peripherals vary a lot.
Different manufacturers may design and develop their own SoCs.
These new SoCs introduce many new peripherals that are not supported
in \code{QEMU} and the open-sourced mainstream of the Linux kernel.
%Apart from the \textit{machine specific code}
%in the main distribution of Linux kernel, manufacturers used to write new
%drivers for their own SoCs for the purpose of customization.
For instance,
%\smallskip
%\noindent
\code{QEMU} supports nearly 50 different ARM devices.
%which include tens of models for each type of peripheral.
However, due to the diversity of peripherals, there are still a
large number of devices that are not supported. 
%To support these machines, the developers should read the specifications of these machines very carefully, which requires a huge number of manual efforts. Furthermore, manufacturers may not release the specifications due to the privacy and security. Without the specification, it is rather hard to build the right model for the machines. 
Thus, the diversity of peripherals brings significant challenge to build a general emulator,
which can re-host various Linux kernels of embedded devices.

\smallskip
\noindent
\textbf{Closed Source}:
The high-level information (e.g., source code, specifications, and datasheets)
of the device
is usually not available. Furthermore, the binary code of the Linux kernel is
stripped and has no particular headers (i.e., ELF section headers) or
debugging information. This brings significant challenges since it is hard to
directly infer
the right peripheral models used by the Linux kernel.


\subsection{Observations}
\label{sec:observation}
Though there are several challenges in re-hosting the Linux kernel of embedded devices,
we have some interesting observations %after studying the Linux kernel and ARM architecture carefully.

\smallskip
\noindent \textbf{We don't need to emulate all the peripherals.}
To re-host the Linux kernel, we do not need to emulate all the peripherals. 
%For example, if we are not interested in the network, we do not need to emulate the related peripherals like the network card. Meanwhile, the initialization process of many peripherals do not disturb the kernel start process. Thus, we need to understand what peripherals are required to make the operating system work during the 
%kernel start process. 
After carefully studying the Linux kernel, we find that 
the IC  and timer are the two key peripherals.
IC is responsible for handling different interrupts.  Peripherals send interrupt signals to inform processors that some events are happening
and should to be handled.
%Without interrupts, the CPU may keep working on the current task
%without task switching. Then all the other peripherals cannot be responded as their
%interrupts are not handled, which can result in deadlock or being stuck.
Timer is responsible for scheduling.
A large number of functions in Linux kernel are time-driven. These functions are
invoked periodically. Without timer, the scheduled events cannot be
triggered. In Linux kernel, every time the timer ticks, the number of ticks,
which is stored in a variable (i.e., \textit{Jiffies}), increases by 1.
If the timer does not work, the Linux kernel gets stuck.

Figure~\ref{fig:calibrate_delay} illustrates 
%one usage of the timer in the kernel.During its boot, 
that the kernel  checks whether the timer works in the
function \textit{calibrate\_delay\_converge} during the boot process. 
If the timer does not work properly, the value of \textit{Jiffies} will keep
unchanged. Then the Linux kernel will get stuck in the infinite loop at line 5. 

\begin{figure}[t]
  \centering
  \adjustbox{scale = 1}{
\begin{lstlisting}[basicstyle=\bfseries\fontsize{7.5}{7.5}\ttfamily, keywordstyle=\bfseries\color{blue}\ttfamily, stringstyle=\color{red}\ttfamily, commentstyle=\color{brown}\ttfamily, language=C, breaklines=true, tabsize=2,  numbers=left, firstnumber = 1, gobble=4]
    unsigned long calibrate_delay_converge(void)
    {
        ...
        ticks = jiffies;
        while (ticks == jiffies)
        ...
    }
\end{lstlisting}
}
\caption{The code snippet of \code{calibrate\_delay\_converge} in Linux kernel.}
\label{fig:calibrate_delay}
\end{figure}

\smallskip
\noindent \textbf{Linux kernel provides interfaces for manufacturers to implement drivers of peripherals.} For example, Linux kernel uses the structure \textit{machine\_desc} to describe different machines, which is mentioned in Section~\ref{sec:arm_machine}. In structure \textit{machine\_desc}, function pointer \textit{machine\_desc$\rightarrow$init\_irq} is the interface to implement the driver of IC. 
%We noticed that the offsets of the two function pointers \textit{init\_irq} and \textit{init\_time} compared with struct \textit{machine\_desc} are fixed. Thus, if we know the offset of the struct \textit{machine\_desc}, we can calculate the offsets of function pointers \textit{machine\_desc$\rightarrow$init\_irq} and \textit{machine\_desc$\rightarrow$init\_time} directly. 
Though different devices have different peripheral drivers for different peripherals, 
this common interface can facilitate the process to replace the diverse peripherals (e.g., IC)
with a general one (\textit{peripheral transplantation}), which can solve the problem of peripheral diversity.

%with binary rewriting technique, we can change the value of the function pointer during the re-hosting process. This observation brings us the chance to replace the diverse peripherals with a general one, which can solve the problem of peripheral diversity.
%to redirect the initialization process of interrupt controller and timer to our self controlled code. If we can control the initialization process of these two peripherals, we can prepare general drivers and peripherals of interrupt controller and timer

\smallskip
\noindent \textbf{The Linux kernel of different devices share most of the source code}. Though high-level information of commercialized embedded devices is not available, these Linux-based firmware images still share the code of Linux kernel, which includes the \code{common code} and the \code{architecture specific code} (Section~\ref{subsec:kernel}). The differences are usually the \code{machine specific code}.
% This makes sense as the developers of these manufacturers do not spend a huge amount of time on writing \code{common code} or \code{architecture specific code}. 
%To port the Linux kernel to support their own products. What they do is to define a \textit{machine\_desc} object and assign the machine-specific functions written by themselves to the related pointers. They can invoke the other functions provided by the Linux kernel directly. 
This makes the use of the domain knowledge of the Linux kernel to identify critical data structures and functions possible.


\subsection{Our Novel Technique: Peripheral Transplantation}
\label{sec:solution}


%Peripheral transplantation requires us to transplant two components, i.e., emulated model
%of the peripheral (into QEMU) and the driver of the peripheral (into the Linux kernel).
%Transplanting the peripheral model requires us to build the hardware emulation code for a
%specified (or simplified) peripheral and integrate it into QEMU.
%We utilize APIs provided by \code{QEMU} for transplanting emulated peripheral models.
%Transplanting the driver into the Linux kernel is non-trivial since we have to guarantee three
%design goals: \emph{First}, the code of the transplanted driver should be position-independent.
%Otherwise, the peripheral transplantation technique is limited by the loading address of
%the transplanted driver. 
%\emph{Second}, the transplanted driver should not affect the memory view of the Linux kernel.
%Otherwise, the memory space storing the transplanted driver could be overwrite by the Linux kernel (since
%the kernel is not aware the existence of the driver), resulting in crashes.
%\emph{Third}, the transplanted driver needs to communicate with the original Linux kernel.
%Otherwise, the transplanted driver cannot be initialized and function properly.


The observations mentioned above inspire us to propose a novel technique called \textit{peripheral transplantation},
which is \textit{device-independent} and does not need the source code of the kernel in the target firmware image.
We implement and integrate the technique into \code{QEMU}, which is the state-of-the-art full-system emulator,
to create a firmware dynamic analysis platform named \sysname. 
Specifically, \textit{peripheral transplantation} requires us to transplant two components,
i.e., emulated model
of the peripheral (into \code{QEMU}) and the driver of the peripheral (into the Linux kernel).
We utilize APIs provided by \code{QEMU} for transplanting emulated peripheral models.
%Specifically, \sysname to transplant two components. One is the model of the peripheral (hardware) while the other one is the driver of the peripheral (software). 
%The peripheral model can be described via the APIs provided by \code{QEMU}. We can develop the peripheral model and integrate it into the model of the target device. Then the hardware part of peripheral transplantation is completed.
%Transplanting the model of the peripheral is not difficult, this is because all the peripheral model are described in C code with proposed APIs by \code{QEMU}. We can develop our customized peripheral model and integrate it into the model of the target machine directly. 
%Meanwhile, if we can transplant the driver of the customized peripheral, we can control both the driver and hardware. In this way, 
%the transplanted peripheral can work and the whole kernel can be rehosted successfully.
However, transplanting the driver into the Linux kernel is non-trivial. We have to achieve three goals.
\begin{itemize}

    \item \textbf {The transplanted driver should be position-independent. }
    The transplanted device driver is a binary object. It contains functions and data structures to
    communicate with the peripheral and the Linux kernel.
    However, for normal device drivers, many of the function pointers or data pointers are hard coded.
    When the drivers are transplanted into the kernel with a different base address, we have to change all the absolute
    addresses in the device driver.
    %Furthermore, the driver needs to communicate with the Linux kernel. This brings challenges. 
%    In case the peripheral transplantation is limited by the transplanted address,
	Thus, we need to carefully design the driver and make it position-independent
	and self-contained to be transplanted at any arbitrary address.
%	to 
%    we have to make the driver self-contained so that it can be transplanted at any arbitrary address. 
%    %Meanwhile, we need to provide general interface so that the driver can communicate with Linux kernels in different versions. 
%    Thus, we have to design the driver carefully.

    %Linux kernel is compiled to be self-contained. To transplant the driver of peripheral, we may break the original control flow of the Linux kernel. Meanwhile, the load address of Linux kernel is fixed in the compiling process.  The driver of the peripheral contains all the required functions and structs. However, we have to design the driver carefully and make it to be able to loaded at any arbitrary address.
     
    \item \textbf{The transplanted driver should not affect the memory view of the Linux kernel.}
    The transplanted driver has to be loaded into the physical memory for execution.
%    However, from the original Linux kernel's point of view, this memory region is not available.
    As a result, if we directly inject the driver into the physical memory pages (that are treated as free
    page by the Linux kernel), the pages could be allocated for other purposes.
    That's because the kernel does not explicitly know the existence of the transplanted driver code in the memory.
    Thus, we need to guarantee that the transplanted driver should reside inside a memory region that
    cannot be affected by the Linux kernel.
    
    
    
%    This part of memory must have read, write, and execute access permissions. 
%    If Linux kernel write or allocate the memory containing the transplanted driver, crash can occur. 
%    Thus, we have to guarantee that the transplanted driver cannot influence the memory view of the Linux kernel. 
    %This is because MMU (Memory Management Unit) is introduced in Linux to manage memories.  (e.g., Linux kernel does not allocate it for other purposes).
 
    \item \textbf{The transplanted driver needs to communicate with the original Linux kernel. } 
    %Linux kernel is compressed, stripped, and has no header information. This brings the challenge on inferring the semantics from the kernel code as we only have the pure bytecode.
    The transplanted driver must be initialized by the Linux kernel. Meanwhile, it needs to invoke
    the utility functions inside Linux kernel to communicate with the peripheral.
    Thus, we need to provide general interfaces for the transplanted driver to communicate with
    the original Linux kernel.
   

\end{itemize}

To achieve the first goal, we propose \code{\sysname Driver}. \code{\sysname Driver} is compiled from one C file and then rewritten statically according to the load address to support the position-independent feature. 
\code{\sysname Driver} is  generated by \code{Driver Generator}, which will be illustrated in detail in Section~\ref{sec:driver_generator}, semi-automatically. 
%We write the source code of \code{\sysname Driver} in one C file and compile it into one object file. 
%Note that the compiled object file's load address is \code{0x0}. Besides, the object file has ELF headers and the section \code{.bss} is not initialized.
%Given the arbitrary load address, we calculate the new pointer values of the data pointers and function pointers in \code{\sysname Driver} and rewrite the corresponding values statically.
%As for the \code{.bss} section, which is not initialized, we initialize it by writing zeros to the whole section statically.
%Furthermore, due to the limitation of the jump range in the \textit{BL Label} instruction, \code{\sysname Driver} may not be able to invoke the functions in the original Linux kernel with direct calls. For the direct calls invoking functions in the Linux kernel, we rewrite them as indirect calls, which can break the limitation of the jump range.
%and set the compiling optimization option as O0. This design helps us to change the function pointers easily. 
%It can break the limitation of the jump range in the \textit{BL Label} instruction, which is used for function call in ARM architecture. 
%We will illustrate  \code{\sysname Driver} in detail in Section~\ref{sec:driver_generator}.



To achieve the second goal, we propose the concept of \code{opaque memory}. 
\code{\sysname Driver} that is loaded into the \code{opaque memory} does not affect the memory view
of the original Linux kernel.
Figure~\ref{fig:opaque_memory} shows how \code{opaque memory} works.
Specifically, Linux kernel maintains the memory mapping between the virtual address and physical address
with the help of the emulated MMU. The emulator walks through the page table to translate
the virtual address to the physical address.
\sysname hijacks the page table walk module in \code{QEMU}. When \code{ECMO} aims to
translate a virtual address to a physical address,
\sysname will check whether the virtual address is in the region of the
\code{opaque memory}. If so, \sysname will use the hijacked page table instead of the
page table specified by Linux kernel.
Meanwhile, we provide read, write, and execute access permissions for the \code{opaque memory}. 
In this case, Linux kernel does not know the existence of the \code{opaque memory}.
When we transplant \code{\sysname Driver} and store it in the \code{opaque memory}, it can work normally
without affecting the memory view of Linux kernel.

 
Note that the \code{opaque memory} can be set at an arbitrary address with arbitrary length.
In \sysname, we set the start address of the \code{opaque memory} as \code{0xd0000000}, which is quite far from the load address of Linux kernel (i.e., \code{0xc0008000}). 
We set the length of the \code{opaque memory} as \code{0x10000}. It is large enough to
load the \code{\sysname Driver}, whose size is around \code{0x7400} bytes on average. 
%The start address of \code{opaque memory} (i.e., \code{0xd0000000}) is chosen to guarantee it does not influence the memory view of the Linux kernel. This is because address \code{0xd0000000} is far from the load address of Linux kernel (\code{0xc0008000}) and this part of address will not be read, write, or allocated by the Linux kernel.
%Furthermore, \sysname can transplant \code{\sysname Driver} to any arbitrary addresses.
%Then we provide the privilege of read, write, and execute for \code{opaque memory}. When we redirect the initialization process to the \code{\sysname Driver} in \code{Opaque Memory}, the code can be executed successfully. 

To achieve the third goal, we propose \code{\sysname Pointers} as a bridge. \code{\sysname Pointers} are used in two places. When we start the Linux kernel, we dynamically rewrite the function pointers to redirect the initialization of the original peripheral driver to our \code{\sysname Driver}. We called the \code{\sysname Pointers} used in Linux kernel as \code{\sysname forward pointers}. Inside the \code{\sysname Driver}, it invokes the APIs provided by the Linux kernel to communicate with the peripheral. We called the \code{\sysname Pointers} used in \code{\code{\sysname Driver}} as \code{\sysname Backward Pointers}. We explain how to identify \code{\sysname Pointers} automatically in Section~\ref{sec:pointer_analyzer}.


\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{figures/architecture.pdf}
	
	\caption{The overall architecture of \sysname.}
	\label{fig:architecture}
\end{figure}

Figure~\ref{fig:architecture} shows how \sysname works.
\sysname receives the Linux kernel, \code{\sysname Driver}, and \code{\sysname Pointers} as the input.
The Linux kernel is the guest software, which is to be rehosted by \sysname. \code{\sysname Pointers} are used to communicate between the Linux kernel and \code{\sysname Drivers}. 
During the re-hosting process, when the Linux kernel is going to initialize the peripheral drivers, \code{\sysname Forward Pointers} redirect the initialization process to \code{\sysname Driver}, which is stored in the \code{Opaque Memory}. Inside \code{\sysname Driver}, \code{\sysname Backward Pointers} is utilized to invoke the functions provided by Linux kernel.
% to configure the transplanted peripheral models.
%Note that \sysname drivers vary across different versions of Linux kernel while the \sysname hardwares keep the same. This is because different versions of Linux kernel provides different hardware access APIs for the drivers.

\begin{figure*}[h]
  \centering
  \includegraphics[width=0.8\linewidth]{figures/architecture_example.pdf}
  \caption{An example of \sysname.}
  \label{fig:arch_example}
\end{figure*}

\subsection{A Concrete Example}
Figure~\ref{fig:arch_example} shows a concrete example.
In this example, \sysname transplants two peripherals (i.e., IC and timer) and successfully rehost
the Linux kernel.


 All Linux kernels invoke the function \textit{start\_kernel} during the initialization process (\ballnumber{1}). Function \textit{start\_kernel} will invoke several different functions including \textit{setup\_arch}, \textit{init\_IRQ}, and \textit{time\_init}.  Function \textit{setup\_arch} will set up some configurations related to the architecture and will also initialize the struct \textit{machine\_desc} via function \textit{setup\_machine\_fdt} (\ballnumber{2}). Function \textit{setup\_machine\_fdt} returns back the pointer value of struct \textit{machine\_desc}. \sysname will set a breakpoint here.  Inside the breakpoint, \sysname will set the \code{\sysname Forward Pointers} to redirect the initialization process of IC and Timer (\ballnumber{3}). 
We calculate the offsets of \textit{init\_IRQ} and \textit{init\_time} by adding specific offsets based on the value of \textit{machine\_desc}. Then we assign the pointer value of \textit{\sysnamenospace\_init\_IRQ} and \textit{\sysnamenospace\_init\_time} to the offsets of \textit{init\_IRQ} and \textit{init\_time}, respectively.  After that, when the Linux kernel invokes function \textit{init\_IRQ}, it will check whether the value of this function pointer is empty or not (\ballnumber{4}). If it is not empty, Linux kernel will invoke the function pointed by this value, which is \textit{\sysnamenospace\_init\_IRQ}.  Inside the function \textit{\sysnamenospace\_init\_IRQ}, it invokes several different kinds of APIs that are related to IC in Linux kernel (\ballnumber{5}). \ We call these APIs \textit{configure\_irq\_APIs}, which are \code{\sysname Backward Pointers} (\ballnumber{8}).  The same logic applies to function \textit{time\_init} (\ballnumber{6}). It will invoke the function \textit{\sysnamenospace\_init\_time}.  Inside the function \textit{\sysnamenospace\_init\_time}, it invokes several different kinds of APIs that are related to timer in Linux kernel (\ballnumber{7}). We call these APIs \textit{configure\_time\_APIs}, which are also the \code{\sysname Backward Pointers}.

After transplanting the \code{\sysname Driver} successfully, the timer can trigger interrupts periodically and the IC can handle the triggered interrupts. Then the Linux kernel will mount the root file system before running the \code{shell} process. We build the root file system with \code{Buildroot}~\cite{buildroot} and feed it to the Linux kernel with the opt \code{-initrd} in \code{QEMU}.





==> modules.tex <==
\section{ECMO Modules}
\label{sec:ecmo_modules}

\begin{figure*}[t]
  \centering
  \includegraphics[width=0.6\linewidth]{figures/sys_modules.pdf}
  \caption{The modules of \sysname.}
  \label{fig:module}
\end{figure*}
As we mentioned in Section~\ref{sec:solution}, \sysname requires \code{\sysname Driver} and
\code{\sysname Pointers} to rehost Linux kernel. In this section, we illustrate how to
extract the required Linux kernel, \code{\sysname Driver}, and \code{\sysname Pointers}.
\sysname consists of four modules. They are  \code{Preprocessor}, \code{Decompressor}, \code{Driver Generator}, and \code{Pointer Analyzer}.

Figure~\ref{fig:module} shows the modules of \sysname and their workflow. 
In step 1, 
\code{Preprocessor} (Section~\ref{sec:preprocessor}) conducts  preprocessing on the proposed firmware image.
It unpacks the provided firmware image and extracts the Linux kernel. The Linux kernel here refers to the kernel image
and the corresponding \code{DTB}. 
In step 2, \code{Decompressor} (Section~\ref{sec:decompressor}) decompresses the Linux kernel by dumping the decompressed Linux kernel during re-hosting process.
In step 3, \code{Driver Generator} (Section~\ref{sec:driver_generator}) generates or selects (if already generated) the suited \code{\sysname Driver} by analyzing the decompressed Linux kernel. This is because Linux kernels in different versions have different APIs to communicate with the peripheral and \code{\sysname Driver} needs to invoke these APIs.
In step 4, \code{Pointer Analyzer} (Section~\ref{sec:pointer_analyzer}) analyzes the decompressed Linux kernel and applies the binary analysis techniques to identify \code{\sysname Pointers}. 

%We will introduce how these modules work in detail in the following sections.

%In the second phase, we first feed the extracted description of the firmware to our database of interrupt controller and timer in step 2.1. Meanwhile, we will feed the generated device tree blob and uimage to the eumulator in step 2.2. After receiving the description, the database will return back the suited interrupt controller and timer with specific kernel information in 3.1. Meanwhile, the emulator would dump the raw bytes of the uimage in step 3.2. Then we will feed the interrupt controller, timer, and the dumped raw bytes to the analyzer in step 4. The analyzer will generate the transplant information in step 5. In the third phase, the transplant information will be feed into our emulator in step 6 and it will build the connection between the uimage, dtb, interrupt controller, and timer. Then the linux kernel will be rehosted successfully and we can get the shell in step 7.

\subsection{Preprocesser}
\label{sec:preprocessor}
\code{Preprocessor} is responsible for unpacking the firmware image automatically. We utilize \code{binwalk}~\cite{binwalk} to walk through the firmware image. As the header formats supported by \code{binwalk} are limited, we patch \code{binwalk} to support more header formats. With \code{binwalk}, we can extract Linux kernel image from the packed firmware image. 
The Linux kernel image is in the compressed \code{zImage} format.
We add the u-boot information on the extracted image to get the \code{uImage}.
%With \code{uImage}, \sysname understands the operating system type and the load address. 
%Meanwhile, \code{binwalk} can also extract the \code{DTB} file. 
%We inject the description of peripherals into \code{DTB} so that \code{\sysname Driver} can configure the peripheral model (hardware) with the description of peripheral in \code{DTB}.
%Furthermore, we clean up the \code{DTB} file in the \code{uImage} by writing zeros and feed
%our customized \code{DTB} file with the option of \code{-dtb} in \code{QEMU}.
%Thus, the \code{uImage} will not use the self-contained \code{DTB} file. Instead it reads the required peripheral information from our customized \code{DTB} file.
%As for the decompressed kernel, we observed that statistically decompressing the Linux kernel is not always right and it is not confident. Thus, we propose \code{Decompressor} to dump the decompressed Linux kernel dynamically.

\subsection{Decompressor}
\label{sec:decompressor}
\code{Decompressor} is responsible for decompressing the Linux kernel automatically. 
%After receiving the \code{uImage} and \code{DTB}, 
%the \code{Decompressor} attempts to re-host the Linux kernel. Note that the Linux kernel cannot be rehosted successfully at this stage. However, the goal of  \code{Decompressor} is just to decompress the Linux kernel. 
We notice that Linux kernel will invoke function \textit{decompress\_kernel} to decompress the compressed kernel.
The first parameter of this function (i.e., \textit{output\_start}) indicates the start address of the decompressed Linux kernel.
The size of the decompressed Linux kernel can be automatically inferred by checking the start of large (i.e., \code{0x100000} bytes) empty memory space (i.e., value is zero) after the function \textit{decompress\_kernel} returns.
%As for the size, %\code{binwalk} would try to decompress the Linux Kernel statically. 
%we use the statically decompressed kernel size as the dumped size. Note that the decompressed kernel size does not need to be accurate.
%Only if it contains our required \code{\sysname pointers}, we can identify the \code{\sysname pointers} with \code{Pointer Analyzer}.
Thus, if we can identify when \textit{decompress\_kernel} is invoked, we can get the first parameter by checking the first register (\code{R0} in ARM) and dump the decompressed Linux kernel successfully.


%value of the CPU register at that point. ARM CPU \code{R0}, which represents the return value of \textit{decompress\_kernel}, indicates the return value of \textit{output\_start}. Then we know where the decompressed kernel stores at.

%To identify when the function \textit{decompress\_kernel} is invoked, we just need to identify the address of \textit{decompress\_kernel}.
We notice that the function \textit{decompress\_kernel} is invoked by the assembly code in the file \textit{arch/arm/boot/compressed/head.S}~in Figure~\ref{fig:hard_code}. We check the assembly code across different kernel versions and find that this snippet of code remains unchanged in Linux kernels in different versions.
With this observation, \code{Decompressor} identifies the the address of instruction \code{BL decompress\_kernel} by strictly comparing the execution trace and the hard coded assembly code. After finding the address of the function \textit{decompress\_kernel}, the value \textit{output\_start} can be identified. 
We can feed the uImage to \code{Decompressor} again and set a breakpoint (i.e., \textit{dump\_kernel}) after the function \textit{decompress\_kernel} finishes. Then we can dump the decompressed Linux kernel at the breakpoint.
%Linux kernel is compressed with specific compression algorithm and then packed with some pre-start scripts. 



\subsection{Driver Generator}
\label{sec:driver_generator}
\code{Driver Generator} is responsible for generating \code{\sysname Driver} semi-automatically. For one kernel version, the \code{\sysname driver} is fixed. However, if the release time between two versions is quite long (i.e., 3.x and 4.x), the functions used to configure peripheral models are not the same. Thus, the \code{\sysname driver} may be different for kernels in different versions. 
In the compiling time, the compiler will inject the kernel version information and the compiler information into the compiled kernel. Meanwhile, there are functions for debugging purpose that will print out the kernel version. Thus, we use the GNU binary utilities \code{strings}~\cite{strings} to dump out all the strings in the kernel. After grepping the specific string (i.e., version), we can find the detail kernel version number. 
Then, we generate the \code{\sysname driver} for the corresponding kernel version. We write driver code in one C file (i.e., \textit{\sysnamenospace\_Driver.c}), which is the only procedure that requires the manually effort, and compile it into one object file (i.e., \textit{\sysnamenospace\_Driver.o}).
Writing driver code in one C file is a one-time effort. To support Linux kernel in new versions, users only need to change the functions that are not supported in the previous Linux kernel version, which can be down in less than one hour.
 

Note that the compiled object file's load address is \code{0x0}. Besides, the object file has ELF headers and the section \code{.bss} is not initialized.
Given the arbitrary load address, \code{Driver Generator} calculate the new pointer values of the data pointers and function pointers in \code{\sysname Driver} and rewrite the corresponding values statically.
As for the \code{.bss} section, which is not initialized, \code{Driver Generator} initialize it by writing zeros to the whole section statically.
Furthermore, due to the limitation of the jump range in the \textit{BL Label} instruction, \code{\sysname Driver}, which is stored in the \code{opaque memory}, may not be able to invoke the functions in the original Linux kernel with direct calls. For the direct calls invoking functions in the Linux kernel, we rewrite them as indirect calls, which can break the limitation of the jump range.
%and set the compiling optimization option as O0. This design helps us to change the function pointers easily. 
%It can break the limitation of the jump range in the \textit{BL Label} instruction, which is used for function call in ARM architecture. 
%We will illustrate  \code{\sysname Driver} in detail in Section~\ref{sec:driver_generator}.
%As the \code{\sysname Driver} is stored in the \code{opaque memory}, the offset of \code{opaque memory} can be quite far from the offset of the load address of Linux kernel. Thus, \code{\sysname Driver} cannot invoke the functions in Linux kernel via direct calls due to the limited range of instruction \code{BL}. In \textit{\sysnamenospace\_Driver.c}, all the invoked functions that are in the Linux kernel are re-written as the indirect calls. 
%We also disabled the optimization when compiling the \textit{\sysnamenospace\_Driver.c} into \textit{\sysnamenospace\_Driver.o}. Thus, all the functions are invoked via indirect calls. 
We also noticed that compilers can do optimization to change the indirect calls into direct calls. Thus, we disable all the optimization flags during the compiling process.
This brings the advantages that we can change the indirect called functions by simply changing the function pointers statistically. For example, 
Figure~\ref{fig:ecmo_driver} shows a snippet of assembly code in \code{\sysname Driver}. At address \code{0x10000}, \code{\sysname Driver} loads the value stored at address \code{0x10050} into register \code{R3}. At address \code{0x10004}, \code{\sysname Driver} calls the function that register \code{R3} points to. After identifying the \code{\sysname Pointers}, we can statistically rewriting the value in \code{0x10050}, which can cover the whole memory space in Linux kernel(i.e., $2^{32}$).

\begin{figure}[t]
    \centering
    \adjustbox{scale = 0.8}{
\begin{lstlisting}[basicstyle=\bfseries\fontsize{7.5}{7.5}\ttfamily, keywordstyle=\bfseries\color{blue}\ttfamily, stringstyle=\color{blue}\ttfamily, commentstyle=\color{brown}\ttfamily, language=Ant, breaklines=true, tabsize=2,  numbers=left, firstnumber = 1, gobble=4,showstringspaces=false]
    0x10000: ldr r3, [pc, #72] 
    0x10004: blx r3
    0x10050: "Pointer value of called function"	     
\end{lstlisting}
    }
\caption{How \code{\sysname Driver} indirectly invokes the functions in Linux kernel.}
\label{fig:ecmo_driver}
\end{figure}


%Note these are one time efforts. Once we create an \code{\sysname Driver} for this kernel version, it can be used for many other kernel versions if the related APIs are not changed. 
%\comments{I may need to introduce how the \sysname driver looks like. How it is communicated with kernel APIs}


%The second phase is to extract the transplant information. Here the transplant information is defined as data pointers and function pointers. As we mentioned before, we would like to transplant our compiled interrupt controller and timer into the original linux kernel. To make the transplanted interrupt controller, timer, and linux kernel communicate successfully, we need to dynamic write the related pointers. Thus, proposed algorithm~\ref{alg:match} to identify the required pointers.

%\subsubection{Rehost}
%With the related pointer information, we can rehost the linux kernel of embedded systems. However, there are still challenges. The linux kernel would manage memories for different processes. The internal logic of memory management is very complex. Thus, if we put the general interrupt controller and timer into the memory region of linux kernel, it would break the original memory mangement system of the linux kernel. To make our mechanism work, we put the general interrupt controller and timer into a memory region, which is called fake memory. This part of memory region is maintained by qemu rather than kernel itselfs. We hook the memory 

\subsection{Pointer Analyzer}
\label{sec:pointer_analyzer}
\code{Pointer Analyzer} is responsible for identifying the \code{\sysname Pointers}, which are the pointer values for specific function pointers, from the decompressed Linux kernel. \code{\sysname Pointers} consist of two types. One is \code{\sysname Forward Pointers}, which are used by the Linux kernel to redirect the initialization process of specific drivers to \code{\sysname Driver}. 
The other type is \code{\sysname Backward Pointers}, which are used by \code{\sysname Driver} to invoke the functions provided by Linux kernel to configure peripheral models. 
\code{\sysname Forward Pointers} are set dynamically during the re-hosting process. This is because we cannot re-write \code{\sysname Forward Pointers} until the Linux kernel is decompressed and loaded into memory. 
%rewrite the original pointers at the fixed point. During the start process of Linux kernel, the pointer of struct \textit{machine\_desc} is not set until the function \textit{setup\_machine\_fdt} is invoked. Function \textit{setup\_machine\_fdt} returns back the pointer of struct \textit{machine\_desc}. Then we can calculate the pointer value of the function pointer \textit{init\_irq} and \textit{init\_time} and write the redirected pointers dynamically.
\code{\sysname Backward Pointers} is set by \code{Driver Generator} statically.
This is because that \code{\sysname Driver} is compiled by ourselves and we know the offsets of \code{\sysname Backward Pointers} that we need to rewrite. Thus, we can statically re-write the \code{\sysname Driver} with \code{\sysname Backward Pointers} once we identify them.
%Thus, we will dynamically rewrite the original pointers with \sysname pointers to make \sysname works.

However, identifying \code{\sysname Pointers} accurately is not easy. The main challenge is that the decompressed Linux kernel is stripped. It has no section headers, and contains thousands of different kinds of functions. Furthermore, the Linux kernel is compiled with different compilers and compiling options, which can result in different binaries. Thus, the algorithm we propose cannot have any assumption on the compiling options or compilers. 

%\smallskip \noindent \textbf{Approach}:
We noticed that \code{\sysname Pointers} are usually \code{architecture specific code} or \code{common code}, which is open-source, rather than \code{machine specific code} (Section~\ref{subsec:kernel}). 
With the source code, we can identify the  \code{\sysname Pointers} from the decompressed Linux kernel with the algorithm (Section~\ref{sec:disassemble}) and the identification strategies  (Section~\ref{sec:identify_pointers}).


\begin{algorithm}[!ht]
\footnotesize
  \SetKwInput{KwInput}{Input}                % Set the Input
  \SetKwInput{KwOutput}{Output}              % set the Output
  \DontPrintSemicolon
  \KwInput{The decompressed Linux kernel $B$; \\
  The source code of ECMO Pointers $F$ (common code or architecture specific code);}
  \KwOutput{The addresses of ECMO Pointers $V$;}

  \SetKwFunction{FIdentify}{Identify}
  \SetKwFunction{FGenerateFunctions}{GenerateFunctions}
  \SetKwFunction{FDisassembly}{Disassembly}

  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FIdentify{$B$,$F$}}{
    CFG = Disassembly($B$)\;
    Generated\_Functions = GenerateFunctions($CFG$)\;
    
    \For(){$R\_F$ in $F$}{
      \For(){$C\_F$ in $Generated\_Functions$}{
      \For(){Filtering\_Strategy in Filtering\_strategies}{
        \If(){Filtering\_Strategy($R\_F$,$C\_F$)}{
          Append $C\_F$ to Candidates of $R\_F$
        }

      }
      }
      }

      \For(){$R\_F$ in $F$}{
      \If(){Length(Candidates of $R\_F$) == 1}{
        Append Candidates to $V$
      }
    }
    \Return V\;
  }
  \;

  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FDisassembly{$B$}}{
    Instructions = LinearDisassembly(B)\;
    CFG = Empty\;
    \For(){Inst in Instructions}{
        BB = new BasicBlock()\;
        \eIf() {Inst is Branch Instruction}{
        Jump\_Target = Get\_Jump\_Target(Inst)\;
        BB.add\_Successor(Jump\_Target)\;
        CFG.add\_BasicBlock(BB)\;
        BB = new BasicBlock()\;
        }
        {
        BB.add\_Inst(Inst)\;
        }
    }
    \Return CFG\;
  }
\;

%\SetKwProg{Fn}{Function}{:}{}
%  \Fn{\FGenerateFunctions{$CFG$}}{
%    Functions = Empty\;
%    BasicBlocks = CFG.BasicBlock\;
%    \For(){BB in BasicBlocks}{
%      \uIf(){FunctionSignature(BB)}{
%        NewFunction = Function(BB.StartAddress)\;
%        Append NewFunction to Functions\;
%      }
%      \uIf(){BB jumped by Instruction BL}{
%        NewFunction = Function(BB.StartAddress)\;
%        Append NewFunction to Functions\;
%      }
%    }
%    \Return Functions
%  }
%  \;

\caption{The algorithm to identify the function addresses from the  decompressed Linux kernel.}
  \label{alg:match}
\end{algorithm}

\subsubsection{Algorithm}
\label{sec:disassemble}
%As we mentioned in Section~\ref{sec:observation}, for a specific version of Linux kernel, drivers share the same functions to communicate with the peripherals. 

The detailed algorithm is described in algorithm~\ref{alg:match}. We have the decompressed Linux kernel (i.e., B), and the source code of \code{\sysname Pointers} (i.e., F). They are \code{architecture specific code} or \code{common code}, which is open-source. The outputs of the algorithm are the addresses of \code{\sysname Pointers} (i.e., V). First, we disassemble the decompressed Linux kernel and generate the control flow graph (line 2). The load address for Linux kernel is usually fixed (i.e., \code{0xc0008000}). 
With the control flow graph, we generate the function boundaries of decompressed Linux kernel (line 3). Then we loop the generated functions (line 4) and apply three filtering strategies (line 6) to each \code{\sysname Pointer} on each generated function. If the filtering strategy (Section~\ref{sec:identify_pointers}) can identify one generated function as a candidate of one \code{\sysname Pointer} (line 7), this function will be appended to the candidate list of the \code{\sysname Pointer} (line 10). 
Finally, we check the candidates of each \code{\sysname Pointer} (line 12). If there is only one candidate, it means this function is identified.

It is well known that accurately disassemble the ARM binaries is still challenging~\cite{jiang2020empirical}, especially when the binary is stripped and has no section headers. Our disassembly algorithm needs to guarantee there are no false negatives. Otherwise, \code{\sysname Pointers} may not be identified due to the disassembly error. False positives are acceptable as the filtering strategies can help us to filter out these false positives. Thus, we use linearly disassembly strategy, which is conservative and has no false negatives.  After disassembling all the instructions, we loop all the instructions (line 19) and check whether this instruction is a branch instruction or not (line 21). Note that if the instruction changes the value of \code{PC} register implicitly, it is also treated as a branch instruction. If the instruction is a branch instruction, we calculate the jump targets (line 22), add the jump targets to the successor of the basic block (line 23), append the basic block into the control flow graph (line 24), and initialize a new basic block (line 25). If it is not a branch instruction, we append the instruction to the basic block directly (line 27).

Identifying the function boundaries is also a challenging task. If we cannot identify the function boundaries accurately, we may fail to identify the \code{\sysname Pointers}. We implement the  state-of-the-art function identification algorithm introduced in \code{Nucleus}~\cite{andriesse2017compiler} for ARM binaries.
%Besides, we also loop all the basic blocks to check whether they have the signature (i.e., push the registers to stack) of a function. If so, it will also be treated as a function.
%Our function generation algorithm is conservative and may have false positives. However, it is acceptable as the filter strategies~\ref{\label{sec:identify_pointers}} can help us to find the final candidate.
%We first treat the jump targets of instruction \code{BL} as functions. We loop all the basic blocks (line 33) and check whether they have the signature (i.e., push the registers to stack) of a function (line 34). If it has the signature, a new function will be created (line 35). Apart from this, some functions may not have the signature due to the optimization of compilers. We would check whether these functions are jumped by instruction \code{BL}, which is widely used in ARM to invoke a function. If it is (line 37), we will also treat it as a new function (line 38).






\subsubsection{Strategies}
\label{sec:identify_pointers}
As we mentioned in algorithm~\ref{alg:match}, we use three filtering strategies to find the addresses of \code{\sysname Pointers}.
We illustrate them in the following.
%Now we will introduce them in detail. 

\smallskip
\noindent \textbf{Strategy One} In this strategy, we mainly focus on two signatures. One is the specific string. In Linux kernel, it is very normal that the functions will print some specific strings. We can check which function has the data reference on this specific string. 
The other one is warning on specific condition. The functions that are used to print out the warning receives two parameters.  The first parameter is the filename that contains the function. The second parameter is the line number of the source code that triggers the warning. The filename can help us to identify all the functions that contain warnings in this file. However, there might be more than one candidate. Thus, we also need to know the line number. We conduct partial emulation for each basic block to identify the line number. Appendix~\ref{appendix:strategy_one_example} shows detailed examples. Strategy One can help us to identify some functions directly.
%Note that the developers used to not change the \code{common code} or \code{architecture specific code}. However, in case developers insert some help functions in the files, which can change the line number, we first check whether there is a function whose first parameter is exactly the same as the line number in source code. If it is, this function can be identified. If we cannot find such a function, we enlarge the scope of the line number. This can help us to identify more than one candidate. Strategy two and three can help us filter out the false positives. 



\smallskip
\noindent \textbf{Strategy Two} Functions that do not contain specific strings or any warnings cannot be identified by strategy one. To identify these functions (i.e., required functions), we consider their relationship with the functions that can be identified (i.e., identified functions). We mainly consider three relationships. They are caller relationship, callee relationship, and sibling relationship. Caller relationship refers to that the required functions called the identified functions. Callee relationship refers to that the identified functions called the required functions. Sibling relationship refers to that some other functions called both the identified functions and required functions. Appendix~\ref{appendix:strategy_two_example} shows detailed examples. Strategy two can help us to identify some functions indirectly.
 


\smallskip
\noindent \textbf{Strategy Three} Even we use the strategy two, we are not able to identify a few functions as one function can have more than one caller, callee, or sibling. Thus, we need to further consider the primitives of the required functions. Strategy three mainly considers three primitives. They are specific value, basic block number, and callee number. For example, if the function contains logic operation on some specific values (e.g., \code{a = a|0x300}). The compiler would compile the source code and generate the assembly code that contains the specific values (e.g., \code{orr r0,r0, \#0x300}). Furthermore, the number of basic blocks and callees are also used to help us to find the right candidate. Appendix~\ref{appendix:strategy_three_example} shows detailed examples. Strategy three can help us to identify the left functions.

With \code{Pointer Analyzer}, we can successfully identify  \code{\sysname Pointers}.
%However, due to the optimization of compilers, the basic block number may not be predicted even we have the source code. In this case, we think a function with more if/else statements is more complex, which should have more basic blocks. Thus, when we only have limited candidates for one function after applying strategy one and strategy two, we know the complexity of these candidates. We can find the one whose basic block number ranks the same as its complexity ranks in the source code.



==> table/overall.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\caption{The overall result of \sysname on re-hosting the Linux kernel of OpenWRT . Success Rate of Transplantation = (Peripherals Transplanted)/(Kernel Extracted); Success Rate of Re-hosting = (Shell)/(Kernel Extracted).}
\vspace{-0.1in}
\scalebox{0.75}{
\begin{tabular}{c|c|c|c|c|c|c|c|c} 
\toprule
Kernel  Version & Images & Format Supported & Kernel Extracted & \begin{tabular}[c]{@{}c@{}}Peripherals \\ Transplanted \end{tabular} & \begin{tabular}[c]{@{}c@{}}Success Rate of\\ Transplantation \end{tabular} & \begin{tabular}[c]{@{}c@{}}Cannot Mount\\ File System \end{tabular} & Shell & \begin{tabular}[c]{@{}c@{}}Success Rate of \\ Rehosting \end{tabular}  \\ 
\hline\hline
3.18.20         & 52     & 52               & 50               & 50                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 16                                                                  & 34    & {\cellcolor[rgb]{0.643,0.863,1}}68\%                                    \\ 
\hline
4.4.50          & 119    & 119              & 111              & 111                                                                   & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 24                                                                  & 87    & {\cellcolor[rgb]{0.643,0.863,1}}78.4\%                                  \\ 
\hline
4.4.61          & 39     & 39               & 37               & 37                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 8                                                                   & 29    & {\cellcolor[rgb]{0.643,0.863,1}}78.4\%                                  \\ 
\hline
4.4.71          & 40     & 40               & 38               & 38                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 8                                                                   & 30    & {\cellcolor[rgb]{0.643,0.863,1}}78.9\%                                  \\ 
\hline
4.4.89          & 40     & 40               & 38               & 38                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 8                                                                   & 30    & {\cellcolor[rgb]{0.643,0.863,1}}78.9\%                                  \\ 
\hline
4.4.92          & 41     & 41               & 38               & 38                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 8                                                                   & 30    & {\cellcolor[rgb]{0.643,0.863,1}}78.9\%                                  \\ 
\hline
4.4.140         & 41     & 41               & 38               & 38                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 8                                                                   & 30    & {\cellcolor[rgb]{0.643,0.863,1}}78.9\%                                  \\ 
\hline
4.4.153         & 40     & 38               & 38               & 38                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 8                                                                   & 30    & {\cellcolor[rgb]{0.643,0.863,1}}78.9\%                                  \\ 
\hline
4.4.182         & 40     & 38               & 38               & 38                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 8                                                                   & 30    & {\cellcolor[rgb]{0.643,0.863,1}}78.9\%                                  \\ 
\hline
4.14.54         & 54     & 54               & 42               & 42                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 0                                                                   & 42    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                   \\ 
\hline
4.14.63         & 66     & 66               & 42               & 42                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 0                                                                   & 42    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                   \\ 
\hline
4.14.95         & 66     & 66               & 42               & 42                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 0                                                                   & 42    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                   \\ 
\hline
4.14.128        & 66     & 66               & 42               & 42                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 0                                                                   & 42    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                   \\ 
\hline
4.14.131        & 66     & 66               & 42               & 42                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 0                                                                   & 42    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                   \\ 
\hline
4.14.151        & 66     & 66               & 42               & 42                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 0                                                                   & 42    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                   \\ 
\hline
4.14.162        & 66     & 66               & 42               & 42                                                                    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 0                                                                   & 42    & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                   \\ 
\hline\hline
Overall         & 902    & 902              & 720              & 720                                                                   & {\cellcolor[rgb]{0.643,0.863,1}}100\%                                       & 96                                                                  & 624   & {\cellcolor[rgb]{0.643,0.863,1}}86.7\%                                  \\
\bottomrule
\end{tabular}
}
\label{tab:overall}
\end{table*}

==> table/pointer.tex <==
\begin{table*}[t]
\centering
\footnotesize
\caption{The \sysname pointers, identification strategy, and the description of these pointers. NA: Not Applicable.}
\scalebox{0.85}{
\begin{tabular}{l|l|l|l|l} 
\toprule
Kernel Version        & \code{\sysname Forward Pointers}                                                                                   & \code{\sysname Backward Pointers}             & Strategy & Description                                                             \\ 
\hline
\hline
\multirow{13}{*}{ALL} & \multirow{15}{*}{\begin{tabular}[c]{@{}l@{}}mach\_desc-init\_irq\\ mach\_desc-init\_time \end{tabular}} & irq\_set\_chip\_and\_handler\_name & III    & Setup the chip and handler of an interrupt request                      \\ 
\cline{3-5}
                      &                                                                                                         & irq\_set\_chip\_data               & III    & Setup the data of the specified chip                                    \\ 
\cline{3-5}
                      &                                                                                                         & handle\_level\_irq                 & II     & Level type irq handler, which is used as the callback function          \\ 
\cline{3-5}
                      &                                                                                                         & \_\_handle\_domain\_irq            & III    & Covert a hardware interrupt number to a logical one using a IRQ domain  \\ 
\cline{3-5}
                      &                                                                                                         & setup\_machine\_fdt                & I      & Setup machine when the dtb is passed to the kernel                      \\ 
\cline{3-5}
                      &                                                                                                         & set\_handle\_irq                   & III    & Generic IRQ handler function, which is the top-level IRQ handler        \\ 
\cline{3-5}
                      &                                                                                                         & irq\_domain\_add\_simple           & III    & Register the IRQ domain                                                 \\ 
\cline{3-5}
                      &                                                                                                         & irq\_create\_mapping               & I      & Map a hardware interrupt into Linux IRQ space                           \\ 
\cline{3-5}
                      &                                                                                                         & of\_find\_node\_by\_path           & II     & Find a device node with specific path                                   \\ 

\cline{3-5}
                      &                                                                                                         & setup\_irq                         & I      & Setup an interrupt                                                      \\ 
\cline{3-5}
                      &                                                                                                         & clockevents\_config\_and\_register & III    & Configure and register a clock event device                             \\ 
\cline{3-5}
                      &                                                                                                         & irq\_domain\_xlate\_onetwocell     & I      & Generic xlate for one or two cell bindings                              \\ 
\cline{3-5}
                      &                                                                                                         & warn\_slowpath\_null               & I      & Warning information                                                     \\ 
\cline{1-1}\cline{3-5}
3.18.x                &                                                                                                         & set\_irq\_flags                    & I      & \multirow{2}{*}{Modify the status of an interrupt request}              \\ 
\cline{1-1}\cline{3-4}
4.4.x / 4.14.x        &                                                                                                         & irq\_modify\_status                & III    &                                                                         \\
\bottomrule
\end{tabular}


\label{tab:pointer}
}
\end{table*}
